Online Linear Optimization with Many Hints

We study an online linear optimization (OLO) problem in which the learner is provided access to $K$ "hint" vectors in each round prior to making a decision. In this setting, we devise an algorithm that obtains logarithmic regret whenever there exists a convex combination of the $K$ hints that has positive correlation with the cost vectors. This significantly extends prior work that considered only the case $K=1$. To accomplish this, we develop a way to combine many arbitrary OLO algorithms to obtain regret only a logarithmically worse factor than the minimum regret of the original algorithms in hindsight; this result is of independent interest.

==> multi.tex <==
\section{Multiple hints}

Suppose in each round instead of getting a single hint $h_t$, we get $K$ hints $h^1_t,\dots,h^K_t$. We'd like to do nearly as well as if we were just given the best sequence of hints: $h^i_1,\dots, h^i_T$.
We consider ``learning the best hint'' by running an online learner on the $K$ hints. This online learner will play weights $w_t=(w^1_t,\dots,w^K_t)$ in the $K-1$-dimensional simplex in $\mathbb{R}^K$. Then, we provide the actual online-learning-with-hints algorithm with the hint $h_t = \sum_{i=1}^K w^i h^i_t$. Our task is to design the $w$-learner such that when it has low regret, the hints it produces are as good as the best hints.


\section{Hinge-Loss approach: this is broken (sketch of potential fix is below in section 6)}
Intuitively, one might consider setting the loss $\ell_t$ experienced by this learner to be $\ell_t(w)=\sum_{i=1}^K\langle c_t, h^i_t\rangle w^i$. However, for some technical reasons this seems like it might not work well. Instead, we will consider a hinge-like loss:
\[
\ell_t(w)=\max\left(0, \alpha - \sum_{i=1}^K\langle c_t, h^i_t\rangle w^i\right)
\]
We'll consider a hint to be $\alpha$-good if $\langle c_t, h_t\rangle \ge \alpha$. Note that this is a more stringent definition of $\alpha$-good than in the icml submission.

This loss has a few important properties:
\begin{enumerate}
\item It is convex (in $w$).
\item It is non-negative.
\item $\ell_t(w) \le 1$ for all $w$ in the simplex.
\item If $h_t = \sum_{i=1}^K w^i h^i_t$ is $\alpha$-good, then $\ell_t(w)=0$ and $0\in \partial \ell_t(w)$.
\item Supposing each $h^i_t$ and $c_t$ satisfy $|\langle c_t, h^i_t\rangle|\le 1$, $\ell_t$ is 1-Lipschitz with respect to the $1$-norm, which means that all subgradients have $\infty$-norm at most 1.
\end{enumerate}

Next, we recall that there exists an OLO algorithm with domain equal to the simplex and regret guarantee:
\begin{align*}
\sum_{t=1}^T\langle g_t, w_t - w_\star\rangle \le \sqrt{\log(K) \sum_{t=1}^T \|g_t\|_\infty^2}
\end{align*}
(to get this, consider the $\log(K)$-norm as an approximation to the $\infty$-norm and use adaptive mirror-descent or FTRL style analysis similar to as in the appendix of the icml submission).

Let us use such an algorithm as the $w$-learner, where we set $g_t\in\partial \ell_t(w_t)$. Then since $\|g_t\|_\infty\le 1$ and $g_t=0$ if $h_t$ is $\alpha$-good, we have that
\begin{align*}
\sum_{t=1}^T \ell_t(w_t)-\ell_t(w_\star)\le \sqrt{\log(K) B}
\end{align*}
where $B$ is the number of time steps when $h_t$ is not $\alpha$-good. 


Suppose that one of the hint sequences has at most $Z$ hints that are not $\alpha$-good. WLOG suppose it is the first one. Let $w_\star=(1,0,\dots,0)$. Then since $\ell_t(w)\le 1$ for all $w$ in the simplex,
\begin{align*}
\sum_{t=1}^T \ell_t(w_\star)\le Z
\end{align*}
Therefore
\begin{align*}
\sum_{t=1}^T \ell_t(w_t)\le \sqrt{\log(K) B} + Z
\end{align*}
Let $M$ be the number of times that $h_t$ is not $\alpha/2$-good. Notice that whenever $h_t$ is not $\alpha/2$ good, we must have $\ell_t(w_t)\ge \frac{\alpha}{2}$. Therefore
\begin{align*}
\sum_{t=1}^T \ell_t(w_t) \ge \frac{\alpha M}{2}
\end{align*}
Thus (noticing that $M\ge B$),
\begin{align*}
\frac{\alpha M}{2} \le \sqrt{\log(K) B} + Z\le \sqrt{\log(K) M}+  Z
\end{align*}
Solving for $M$, and being very loose with the constants, this implies:
\begin{align*}
M\le \frac{4Z}{\alpha} + \frac{16 \log(K)}{\alpha^2}
\end{align*}

Recall that the original bound in the icml submission, if we just used the hint sequence $h^1_t$ that has only $Z$ hints that are not $\alpha$-good, gets regret:
\begin{align*}
\tilde O\left(\frac{\sqrt{Z}}{\alpha}\right)
\end{align*}

If we use instead the hints $h_t=\sum_{i=1}^K w^i h^i_t$, we have $M$ hints are not $\alpha/2$-good, so the regret is:
\begin{align*}
\tilde O\left(\frac{\sqrt{Z}}{\alpha^{3/2}} + \frac{\sqrt{\log(K)}}{\alpha^2}\right)
\end{align*}

Some things to improve here:
\begin{itemize}
    \item The notion of $\alpha$-good here is weaker than the the icml submission.
    \item The dependence on $\alpha$ is wrong.
    \item We need to choose an $\alpha$ up-front in order to set the losses for $w_t$-learner.
\end{itemize}

Some dependence on $\sqrt{\log(K)}$ is probably unavoidable (but the $1/\alpha^2$ may not be tight): consider a 1-D problem where there are $K=2^T$ sequences of hints, one for every possible length-$T$ sequence of $\pm 1$. Let the $c_t$ be a sequence of random signs. Then clearly the algorithm must suffer $\sqrt{T}=\sqrt{\log(K)}$ regret even though there is definitely one hint sequence that is actually equal to the loss sequence.

\subsection{If all experts are always good}
Say expert $i$ gives hints that are always at least $\alpha_i$ good, i.e. $\langle c_t, h_t^i\rangle \geq \alpha_i,\ \forall t$. Our algorithm does not know any $\alpha_i$.

It's easy to get regret $O(\dfrac{\log T}{\alpha})$ where $\alpha = \max_i \alpha_i$.

\subsection{Unconstrained Domain}

The old algorithm actually works directly (hopefully). Still need to do the analysis.

\subsection{Standard MWU on hints}
Suppose we have $K$ hints $h_t^i$ at each step $t$, $1 \le i\le K$. If we know $\alpha$, we can simply define binary losses for the hint players, using:
\[\ell_{t, i} = \begin{cases} 0~~ \text{ if } |\iprod{c_t, h_t^i}| \ge \alpha \norm{c_t}, \\ 1 ~~\text{ otherwise.} \end{cases}. \]

Now, simply run a multiplicative weight update algorithm on these hint players. Then by the standard analysis (e.g., Theorem 2.1 of the Arora et al. survey), if $\eta$ is the decay factor used, we have
\[ \E[ \text{regret} ] \le \frac{\log K}{\eta} + \eta \left(\sum_t \ell_{t, i^*}^2 \right). \]

For the best expert, the term in the parenthesis is at most $Z$. Setting $\eta$ appropriately, we get that the expected regret is at most $\sqrt{Z \log K}$.

The regret bound (since the losses of the algorithm are also binary) simply means that the expected number of steps in which the MWU algorithm chooses a bad expert is at most $Z + \sqrt{Z \log K}$. Using our old result, we get the regret of the ``outer'' algorithm to be at most
\[ \frac{ (Z + \sqrt{Z \log K})^{1/2}}{\alpha} \le \frac{2Z^{1/2} + (\log K)^{1/2}}{\alpha}.    \]
In fact, perhaps we could have chosen $\eta = 1/2$ in the MWU step and still be OK.

\section{Single Hint - Strong Regret}

Consider the following stronger notion of regret - For any time interval $[t_1, t_2]$, suppose we want to guarantee small regret with the best fixed expert over that time interval.

In the model of a single hint, say with all hints being promised to be good, can we get $\log (t_2 - t_1)$ regret? If we have $Z$ bad hints in the interval, can we get $\sqrt{Z}$ regret?

\section{All Good Hints}
Suppose all hints are non-negatively correlated. Let us use the hint $h_t = \sum_{i=1}^K w_{t}^ih_{t}^i$, and select $w_t$ via an OLO algorithm with domain equal to the $K$-simplex on the losses
\begin{align*}
    \ell_t(w) = -\sum_{i=1}^k \langle c_t, h_t^i\rangle w^i
\end{align*}
Since $w_t^i\ge 0$ for all $i$ and $t$ and $\langle c_t, h_t^i\rangle\ge 0$ for all $i$ and $t$, we have $\langle c_t, h_t\rangle \ge 0$ for all $t$ - there are no anti-correlated hints.



Let $w_\star$ be an arbitrary element of the simplex. Define $h_t^\star = \sum_{i=1}^K h_t^i w_\star^i$. Then if we choose $w$ using multiplicative weights, we have the guarantee for any $\tau$:
\begin{align*}
    \sum_{t=1}^\tau \ell_t(w_t) - \ell_t(w_\star)&\le  \frac{\log(K)}{\epsilon} + \epsilon \sum_{t=1}^\tau \langle c_t, h_t^\star\rangle 
\end{align*}
Set $\epsilon = \frac{1}{2}$ to obtain:
\begin{align*}
    \sum_{t=1}^\tau \langle c_\tau, h_\tau\rangle \ge   \frac{1}{2}\sum_{t=1}^\tau \langle c_t, h_t^\star\rangle - 2\log(K)
\end{align*}

From the regret analysis in the icml paper, if we use the hints $h_t$, the regret will be bounded by:
\begin{align*}
    R&\le \inf_{\lambda} \lambda + \sum_{t=1}^T \frac{\|c_t\|^2}{\lambda + \sum_{\tau=1}^t \langle c_\tau, h_\tau\rangle }\\
    &\le \inf_{\lambda} \lambda + \sum_{t=1}^T \frac{\|c_t\|^2}{\lambda +  \frac{1}{2}\sum_{t=1}^\tau \langle c_t, h_t^\star\rangle - 2\log(K) }
\end{align*}
Let $Q=\sum_{t| \langle c_t,h_t^\star\rangle <\alpha \|c_t\|^2}\|c_t\|^2$. Let $\lambda = 2\log(K) + \sqrt{Q}$. Then following the analysis in the ICML paper we have regret is bounded by:
\begin{align*}
    O\left(\log(K) + \sqrt{Q} + \frac{\log(T)}{\alpha}\right)
\end{align*}

\begin{itemize}
    \item It might be that better analysis can improve the $\log(K)$ to $\sqrt{\log(K)}$
\end{itemize}









\section{Smoothed Hinge Loss (fixed version of original hinge loss argument)}
Let us consider the following smoothed version of the hinge loss:
\begin{align*}
    \ell(x) = \left\{\begin{array}{lr}
    0& x>\alpha\\
    \frac{1}{\alpha}(\alpha-x)^2& x\in[0,\alpha]\\
    \alpha - 2x& x<0\end{array}\right.
\end{align*}
Then define the $t$th loss $\ell_t$ as:
\[
\ell_t(w)=\ell\left(\sum_{i=1}^K\langle c_t, h^i_t\rangle w^i\right)
\]
We'll consider a hint to be $\alpha$-good if $\langle c_t, h_t\rangle \ge \alpha$. Note that this is a more stringent definition of $\alpha$-good than in the icml submission.

This loss has a few important properties:
\begin{enumerate}
\item It is convex (in $w$).
\item It is non-negative.
\item $\ell_t(w) \le 3$ for all $w$ in the simplex.
\item If $h_t = \sum_{i=1}^K w^i h^i_t$ is $\alpha$-good, then $\ell_t(w)=0$ and $0\in \partial \ell_t(w)$.
\item Supposing each $h^i_t$ and $c_t$ satisfy $|\langle c_t, h^i_t\rangle|\le 1$, $\ell_t$ is 2-Lipschitz with respect to the $1$-norm, which means that all subgradients have $\infty$-norm at most 2.
\item $\ell(x)$ is $\frac{2}{\alpha}$-smooth, so that $\ell'(x)^2\le \frac{4}{\alpha}\ell(x)$. In particular, $\|\nabla \ell_t(w)\|_\infty^2 \le \ell'\left(\sum_{i=1}^K\langle c_t, h^i_t\rangle w^i\right)^2\le \frac{4}{\alpha}\ell_t(w)$.
\end{enumerate}

Next, we recall that there exists an OLO algorithm with domain equal to the simplex and regret guarantee:
\begin{align*}
\sum_{t=1}^T\langle g_t, w_t - w_\star\rangle \le \sqrt{\log(K) \sum_{t=1}^T \|g_t\|_\infty^2}
\end{align*}
(to get this, consider the $\log(K)$-norm as an approximation to the $\infty$-norm and use adaptive mirror-descent or FTRL style analysis similar to as in the appendix of the icml submission). Let us use such an algorithm as the $w$-learner, where we set $g_t\in\partial \ell_t(w_t)$.

Now, observe that $g_t^i\le \langle c_t, h^i_t\rangle \ell'\left(\sum_{i=1}^K\langle c_t, h^i_t\rangle w_t^i\right)$, so that by smoothness:
\begin{align*}
    \|g_t\|_\infty^2 &\le \|c_t\|_2^2 \ell'\left(\sum_{i=1}^K\langle c_t, h^i_t\rangle w_t^i\right)^2\\
    &\le \frac{4}{\alpha}\|c_t\|_2^2 \ell\left(\sum_{i=1}^K\langle c_t, h^i_t\rangle w_t^i\right)\\
    &=\frac{4}{\alpha}\|c_t\|_2^2\ell_t(w_t)
\end{align*}
From this we obtain:
\begin{align*}
    \sum_{t=1}^T \ell_t(w_t) -\ell_t(w_\star)&\le \sqrt{\frac{4\log(K)}{\alpha}\sum_{t=1}^T \|c_t\|_2^2\ell_t(w_t)}\\
    &\le 2\sqrt{\frac{\log(K)}{\alpha}\sum_{t=1}^T\ell_t(w_t)}\\
    &\le 2\sqrt{\frac{\log(K)}{\alpha}\sum_{t=1}^T\ell_t(w_t)-\ell_t(w_\star)}+2\sqrt{\frac{\log(K)}{\alpha}\sum_{t=1}^T\ell_t(w_\star)}
\end{align*}
Then solving for $\sum_{t=1}^T\ell_t(w_t)-\ell_t(w_\star)$ and being loose with constants we obtain:
\begin{align*}
    \sum_{t=1}^T\ell_t(w_t)-\ell_t(w_\star)&\le \frac{16\log(K)}{\alpha}+4\sqrt{\frac{\log(K)}{\alpha}\sum_{t=1}^T\ell_t(w_\star)}\\
    \sum_{t=1}^T\ell_t(w_t)&\le \sum_{t=1}^T \ell_t(w_\star)+\frac{16\log(K)}{\alpha}+4\sqrt{\frac{\log(K)}{\alpha}\sum_{t=1}^T\ell_t(w_\star)}\\
    &\le 2\sum_{t=1}^T \ell_t(w_\star) + \frac{32\log(K)}{\alpha}
\end{align*}

Now, observe that since $\ell_t(w_\star)=0$ if $\langle c_t, \sum_{i=1}^K h^i_t w_\star^i\rangle \ge \alpha$, and $\ell_t(w_\star)\le 3$, we have
\begin{align*}
    2\sum_{t=1}^T \ell_t(w_\star)&\le 6Z
\end{align*}
where $Z$ is the number of times the $w_\star$ weighting produces a hint that is not $\alpha$-good.

Now, notice that we have
\begin{align*}
    \max(0, -\langle c_t, \sum_{i=1}^K h^i_tw^i_t\rangle &\le \ell_t(w_t)
\end{align*}
Therefore if we define $h_t = \sum_{i=1}^K h^i_tw^i_t$, we have
\begin{align}
    \sum_{t=1}^T \max(0, -\langle c_t, h_t\rangle) &\le 6Z + \frac{32\log(K)}{\alpha}\label{eqn:bad}
\end{align}
Let $B=\sum_{t=1}^T \max(0, -\langle c_t, h_t\rangle)$.

Further, if $h_t= \sum_{i=1}^K h^i_t w^i_t$ is not $\alpha/2$ good, we must have $\ell_t(w_t)\ge \frac{\alpha}{4}$. Therefore if $Q$ is the number of times $h_t$ is not $\alpha/2$ good, we have:
\begin{align}
    \frac{\alpha}{4}Q &\le 6Z + \frac{32\log(K)}{\alpha}\nonumber\\
    Q&\le \frac{24Z}{\alpha} + \frac{128\log(K)}{\alpha^2}\label{eqn:Q}
\end{align}
Recall that the original bound in the icml submission, if we just used a hint sequence $h_t$ that has only $Q$ hints that are not $\alpha/2$-good, gets regret:
\begin{align*}
\tilde O\left(\sqrt{Q} + \frac{\sqrt{\sum_{t=1}^T \max(0, -\langle c_t, h_t\rangle)}}{\alpha}\right)
\end{align*}

Thus using our hint sequence $h_t=\sum_{i=1}^K w^i h^i_t$, by (\ref{eqn:bad}) and (\ref{eqn:Q}), the regret is:
\begin{align*}
\tilde O\left(\frac{\sqrt{Z}}{\alpha} + \frac{\sqrt{\log(K)}}{\alpha^{3/2}} \right)
\end{align*}
where again, $Z$ is the number of times that the best linear combination $w_\star$ is not $\alpha$-good.

If we use the improved analysis that gets $\tilde O\left(\sqrt{Q} + \frac{\sqrt{\sum_{t=1}^T \max(0, -\langle c_t, h_t\rangle)}}{\sqrt{\alpha}}\right)$, this improves to
\begin{align*}
\tilde O\left(\frac{\sqrt{Z}}{\sqrt{\alpha}} + \frac{\sqrt{\log(K)}}{\alpha} \right)
\end{align*}

\begin{itemize}
    \item This is still a bit worse than MW in the dependence on $K$. However, it allows for arbitary linear combinations.
\end{itemize}

\section{Lower Bounds}
\begin{theorem}
For any $\alpha$ and $T\ge \frac{\log(1/\alpha)}{\alpha}$, for any online learner, there exists a sequence of $T$ costs and $K$ hints for some $K$ such that there is a convex combination of the $K$ hints that always has correlation $\alpha$ with the costs, but the regret of the learner is at least $\frac{\sqrt{\log(K)}}{\sqrt{2\alpha}}$
\end{theorem}
\begin{proof}
Consider a one-dimensional problem with $K=\frac{T2^B}{B}$ hint sequences for $B=\alpha T$. Suppose $T\ge \frac{\log(1/\alpha)}{\alpha}$, so that $2^B\ge \frac{T}{B}$ and $\log(K)\le 2B=2T\alpha$. We group the hint sequences into $\frac{T}{B}$ groups of size $2^B$. Let us specify the hint sequence in the $i$th such group for some arbitrary $i$. All hints $h_{i,t}$ in the $i$th group are 0 for all $t\notin [(i-1)B,iB-1]$. During these $B$ iterations, the hints take on the $2^B$ possible sequences of $\pm1$. Then it is clear that for \emph{any} sequence of $\pm1$ costs, there is a convex combination of hints that places weight $B/T$ on exactly one hint sequence in each of the $T/B$ groups such that the linear combination always has correlation $\alpha=B/T$ with the cost. 

Let the costs be random signs, so that the expected regret is at $\sqrt{T}$. Then we conclude by observing $\sqrt{\log(K)}/\sqrt{2\alpha}\le \sqrt{2\alpha T}/\sqrt{2\alpha}=\sqrt{T}$.
\end{proof}


This next bound is a bit annoying because it uses $\sum_{t=1}^T \max(0, -\langle c_t, h_t\rangle)$ (which is in fact the term that shows up in our upper-bound) rather than actually having a count of bad hints.
\begin{theorem}
Consider a 2-dimensional problem with $c_t=(\pm \alpha, \pm\sqrt{1-\alpha^2})$, which each sign chosen uniformly at random. Let $h_t = (1,0)$ for all $t$. Then $\E[\sum_{t=1}^T \max(0, -\langle c_t, h_t\rangle)]=\alpha T/2$ and the expected regret of any algorithm is at least $\frac{\sqrt{\E[\sum_{t=1}^T \max(0, -\langle c_t, h_t\rangle)]}}{\sqrt{\alpha}}$.
\end{theorem}
\begin{proof}
A quick computation verifies $\E[\sum_{t=1}^T \max(0, -\langle c_t, h_t\rangle)]=\alpha T/2$. Since $\E[c_t]=0$, the expected cost of the algorithm is $0$. But $\E[\|\sum_{t=1}^T c_t\|] = \sqrt{T}$, so that the expected regret is $\sqrt{T}$.
\end{proof}

Also, the stronger bounds depending on average correlation rather than total number of bad hints we got in unconstrained case actually require a worse dependence on $\alpha$:

\begin{theorem}
In the 1-dimensional unconstrained setting, for any algorithm there is a sequence of costs and 2 sequences of hints that on average one sequence of hints has average correlation $1/\sqrt{T}$ with the costs, but the regret must be at least $R(u)\ge \|u\|\sqrt{T}=\|u\|/\alpha$.
\end{theorem}
\begin{proof}
Let both the costs be independent uniform random signs. Let the first sequence of hints also be random signs, and let the second sequence be $-1$ times the first sequence. Clearly the expected regret must be $R(u)\le \|u\|\sqrt{T}$, but also the expected correlation of the best hint sequences if $1/\sqrt{T}$.
\end{proof}

This actually leaves open how to get the $1/\sqrt{\alpha}$ in the unconstrained setting - presumably while sacrificing the average correlation improvement.

The following simple example shows that even in the single-hint case, when each hint has at least $\alpha$ correlation, the regret is $\Omega(1/\alpha)$.

\begin{theorem}
There exists a sequence of hints $h_t$ and costs $c_t$ in $\R^2$ such that for each $t$, $\iprod{h_t, c_t} \ge \alpha$, and the regret of any online algorithm is $\Omega(1/\alpha)$. // quantifiers reversed 
\end{theorem}
\begin{proof}
Let $e_0$ and $e_1$ be orthogonal unit vectors, and let $h_t = e_0$ for all $t$. Suppose that $c_t = \alpha e_0 \pm \sqrt{1-\alpha^2} e_1$ for all $t$, where the sign is chosen u.a.r. 

Any online algorithm has expected reward at most $\alpha T$ (it cannot gain anything in the $e_1$ direction, so it is best to place all the mass along $e_0$).

On the other hand, the total length $c_{1:t}$ satisfies
\[ \mathbb{E} [\norm{c_{1:t}}^2 ] = \alpha^2 T^2 + T (1-\alpha^2),  \]
and thus the optimal vector in hindsight achieves a reward of $\sqrt{\alpha^2 T^2 + T(1-\alpha^2)}$. Thus the regret is
\[ \frac{T (1-\alpha^2)}{\alpha T + \sqrt{\alpha^2 T^2 + T(1-\alpha^2)}} \ge \frac{T (1-\alpha^2)}{2\alpha T + \sqrt{T(1-\alpha^2)}}. \]
As long as $\alpha < 1$ and $T$ is large enough, this quantity is $\Omega(1/\alpha)$.
\end{proof}

\section{Combining Learners}

We need the following definition of a ``increasing regret bound'':
\begin{defn}
An online learning algorithm $A$ with domain $X$ is associated with an \emph{increasing regret bound} $R(a,b,c_1,\dots,c_T)$ if $R$ is such that when $A$ is run on only the costs $c_a,\dots,c_b$, producing outputs $x_a,\dots,x_b$, we have the guarantee:
\begin{align*}
    \sup_{u\in X}\sum_{t=a}^{b} \langle c_t, x_t\rangle -\langle c_t, u\rangle \le  R(a,b,c_1,\dots,c_T)
\end{align*}
and further, $R$ satisfies the ``increasing property'' $R(a,b, c_1\dots,c_T)\le R(a',b',c_1,\dots,c_T)$ for all sequences $c_t$ whenever $[a,b]\le [a',b']$.
\end{defn}

Basically every worst-case regret bound I am aware of is an increasing regret bound.

Now we can build an algorithm that combines increasing regret bounds. Suppose $A_1,\dots,A_K$ are online learners with corresponding increasing regret bounds $R_1,\dots,R_K$. We will build an online learner that will guarantee the regret bound $2K+2K\min_{i} R_i(1,T, c_1,\dots,c_T)$ for any sequence of costs. We will assume that for all costs $c_t$, $\sup_{x,y\in X}\langle c_t, x-y\rangle\le Z$. $Z$ shows up only in analysis: the algorithm does not need to know it. In the typical case, we should expect $Z=O(1)$.

Intuitively, our scheme is the following: we maintain a guess $\gamma$ for $\min_{i} R_i(1,T, c_1,\dots,c_T)$. Then, we start running algorithm $A_1$. We monitor its worst-case regret $\sup_{u\in X}\sum_{t'=1}^t\langle c_{t'}, x_{t'}- u\rangle$ at all times $t$. Supposing that $R_1(1,T, c_1,\dots,c_T)$ is indeed less than $\gamma$, this value will always be less than $\gamma$ (by the increasing property of $R_1$). If at any point it is \emph{not} less than $\gamma$, we initialize $A_2$ and start running it from then on. We again monitor the worst case regret of $A_2$ over the interval we have been running it on. Again, by the increasing property, if $R_2(1,T, c_1,\dots,c_T)\le \gamma$, this worst-case regret will always be at most $\gamma$. If it ever is not, we switch to $A_3$, and so on. Thus if $\gamma$ is a correct bound, we will never discard the correct algorithm. What is the regret in this case? We only discard an algorithm when it has worst-case regret at most $\gamma+Z$, and if $\gamma$ is correct we never discard the best algorithm, so our final regret is at most $KZ+K\gamma$.

Now what we go through all $K$ algorithms and reject them all? This can only happen if $\gamma$ is incorrect. In this case, we double $\gamma$ and restart the algorithm. If we start with $\gamma=1$, we will only double $\gamma$ at most $\log(TZ)$ times (because we might as well assume all the $R_i\le TZ$). Further, in each round of incorrect $\gamma$, we suffer regret at most $KZ+K\gamma$ so that if $2^M\le 2\min_{i} R_i(1,T, c_1,\dots,c_T)$ is the minimum power of 2 greater than $\min_{i} R_i(1,T, c_1,\dots,c_T)$, overall the regret is at most $\sum_{i=0}^{M} KZ+K2^i\le KM + 2K2^M\le KZ\log(TZ) + 4K\min_{i} R_i(1,T, c_1,\dots,c_T)$.

Note that for many constraint sets, the quantity $\sup_{u\in X}\sum_{t'=1}^t\langle c_{t'}, x_{t'}- u\rangle$ can be efficiently maintained, so that the total complexity of this algorithm is only $O(1)$ time and space per update.

The algorithm is formally described in Algorithm \ref{alg:combiner}.

\begin{algorithm}
\caption{Combiner}\label{alg:combiner}
\begin{algorithmic}
   \STATE{\bfseries Input: } Online learning algorithms $A_1,\dots,A_K$
   \STATE Initialize $A_1$.
   \STATE Set $i=1$, $\gamma=1$, $r=0$, $\tau=1$
   \FOR{$t=1\dots T$}
   \STATE Get $w_\tau$ from $A_i$ and play $x_t=w_\tau$.
   \STATE Get cost $c_t$, define $g_\tau = c_t$.
   \STATE Send $g_\tau$ to $A_i$ as $\tau$th cost.
   \STATE Set $r= \sup_{u\in X}\sum_{\tau'=1}^\tau \langle g_{\tau'}, w_{\tau'}- u\rangle$.
   \IF{$r>\gamma$}
   \IF{$i\ne K$}
   \STATE Set $i=i+1$.
   \STATE Set $\tau=1$.
   \STATE (Re-)Initialize $A_i$.
   \ELSE
   \STATE Set $i=1$.
   \STATE Set $\tau=1$.
   \STATE (Re-)Initialize $A_i$.
   \STATE Set $\gamma = 2\gamma$
   \ENDIF
   \ENDIF
   \ENDFOR
\end{algorithmic}
\end{algorithm}


\subsection{applications}
\begin{enumerate}
    \item Unknown $\alpha$: for any given $\alpha$, our regret bounds are increasing regret bounds. Further, the bound for $\alpha/2$ is only a constant factor away from the bound for $\alpha$. So by maintaining $\log(T)$ different candidate $\alpha$ values we can combine them all to obtain within an $O(\log(T))$ factor of the best possible $\alpha$ value.
    \item Adapting to different norms. For any $\ell_p$ norm for $p\in(1,2]$ there is an algorithm that guarantees regret $\sup_{u\in X} \frac{\|u\|_p}{\sqrt{p-1}} \sqrt{\sum_{t=1}^T \|c_t\|_q^2}$. It may not be clear which $p$-norm is best until we have seen all the costs.  This is an increasing regret bound, so by making a discrete grid of $O(\log(d))$ $p$-norms in a $d$-dimensional space, we can obtain the best of all these bounds in hindsight up to a $\log(d)$ increase.
    \item Adagrad and dimension-free bounds simultaneously. A simple adaptive OGD obtains the regret bound $D_2\sqrt{\sum_{t=1}^T \|c_t\|_2^2}$, where $D_2$ is the 2-norm diameter of $X$. Adagrad instead obtains the bound $D_\infty \sum_{i=1}^d \sqrt{\sum_{t=1}^T c_{t,i}^2}$ where $D_\infty$ is the $\ell_\infty$ diameter of $X$ and $c_{t,i}$ is the $i$th component of $c_t$. The Adagrad bound can be extremely good when the $c_t$ are sparse, but might be much worse than the adaptive OGD bound otherwise. Both are increasing bounds though, so we can combine to get the best of either.
\end{enumerate}


\section{Unconstrained}

\begin{itemize}
    \item TL;DR: there is an unconstrained algorithm that gets regret:
    \begin{align*}
        R_T(u) &= O\left(\frac{\|u\|\log(T)\sqrt{\log(K)}}{\alpha} + \frac{\|u\|\log(T)\sqrt{B}}{\sqrt{\alpha}}\right)
    \end{align*}
    where $\tilde O$ hides constants and log factors in $T$ only. The algorithm does not need to know $\alpha$. The algorithm competes with the best convex combination of the hints.
\end{itemize}
All constants and many logs dropped here in order to keep the math more sane.


Instantiate one $d$-dimensional learner that outputs $x_t$, gets costs $c_t$ and guarantees regret for some user-specified $\epsilon$:
\begin{align*}
    \sum_{t=1}^T \langle c_t, x_t -u\rangle \le \epsilon + \|u\|\sqrt{\sum_{t=1}^T \|c_t\|^2\log(T/\epsilon)}
\end{align*}

Also, instantiate $K$ 1-dimensional learners, one for each hint sequence $h^i_t$. The $i$th such learner outputs $y^i_t$, gets cost $-\langle c_t, h^i_t\rangle$ and guarantees regret:
\begin{align*}
    \sum_{t=1}^T \langle c_t, h^i_t\rangle(y^i - y^i_t)&\le \epsilon/K + |y^i|\sqrt{\sum_{t=1}^T \langle c_t, h^i_t\rangle^2\log(K/\epsilon)}\\
    &\le  \epsilon/K + |y^i|\sqrt{\sum_{t=1}^T \|c_t\|^2\log(KT/\epsilon)}
\end{align*}
(get this algorithm from the previous one by setting $\epsilon\to\epsilon/K$).

We play the predictions $\hat x_t = x_t - \sum_{i=1}^K y^i_t h^i_t$ and set $\epsilon=1$. the regret is:
\begin{align*}
    \sum_{t=1}^T \langle c_t, \hat x_t - u\rangle &\le \inf_{y_i\in \R}\sum_{t=1}^T \langle c_t, x_t -u\rangle+\sum_{i=1}^K\sum_{t=1}^T \langle c_t, h^i_t\rangle(y^i - y^i_t) - \sum_{t=1}^T \langle c_t, \sum_{i=1}^Ky^ih^i_t\rangle\\
    &\le\inf_{y_i\in \R}1 + \|u\|\sqrt{\sum_{t=1}^T \|c_t\|^2\log(T)} + \sum_{i=1}^K\left[1/K + |y^i|\sqrt{\sum_{t=1}^T \|c_t\|^2\log(KT)}\right] -\sum_{t=1}^T \langle c_t, \sum_{i=1}^Ky^ih^i_t\rangle\\
    &\le 2 + \inf_{\sum_i |y_i|\le \|u\|\frac{\sqrt{\log(T)}}{\sqrt{\log(KT)}}}2\|u\|\sqrt{\sum_{t=1}^T \|c_t\|^2\log(T)} -\sum_{t=1}^T \langle c_t, \sum_{i=1}^Ky^ih^i_t\rangle
\end{align*}
Now for any convex combination $h^* = \sum_i w^i h^i$ and any $\alpha\in(0,1]$, let $B_{T,\alpha}$ be defined as in the icml paper, $B_{T,\alpha}$ be a smallest set of indices such that $\sum_{t\notin B_{T,\alpha}} \langle c_t, h^*_t\rangle \ge \alpha\sum_{t\notin B_{T,\alpha}} \|c_t\|^2$. Then set $y^i = \|u\|\frac{w^i}{\sqrt{\alpha |B_{T,\alpha}|+\frac{\log(KT)}{\log(T)}}}$. Notice that $\sum |y^i|\le \|u\|\frac{\sqrt{\log(T)}}{\sqrt{\log(KT)}}$. Also, we have
\begin{align*}
    -\sum_{t=1}^T \langle c_t, h^*_t\rangle&\le -\sum_{t=1}^T \alpha \|c_t\|^2 +2|B_{T,\alpha}|\\
    -\sum_{t=1}^T \langle c_t, \sum_{i=1}^Ky^ih^i_t\rangle&\le -\frac{\|u\|}{\sqrt{\alpha |B_{T,\alpha}|+\frac{\log(KT)}{\log(T)}}}\sum_{t=1}^T \alpha \|c_t\|^2 +2\|u\|\frac{\sqrt{|B_{T,\alpha}|}}{\sqrt{\alpha}}
\end{align*}
Thus overall our bound is:
\begin{align*}
    R_T(u)&\le 2 + 2\|u\|\sqrt{\sum_{t=1}^T \|c_t\|^2\log(T)} -\frac{\|u\|}{\sqrt{\alpha |B_{T,\alpha}|+\frac{\log(KT)}{\log(T)}}}\sum_{t=1}^T \alpha \|c_t\|^2 +2\|u\|\frac{\sqrt{|B_{T,\alpha}|}}{\sqrt{\alpha}}\\
    &\le 2\epsilon + \frac{\|u\| \log(T)\sqrt{\alpha |B_{T,\alpha}|+\frac{\log(KT)}{\log(T)}}}{\alpha} +2\|u\|\frac{\sqrt{|B_{T,\alpha}|}}{\sqrt{\alpha}}\\
    &=O\left(\frac{\|u\|\sqrt{\log(KT)\log(T)}}{\alpha} + \frac{\|u\|\log(T)\sqrt{|B_{T,\alpha}|}}{\sqrt{\alpha}}\right)
\end{align*}
where we set $\epsilon=1$ in the last line.

\begin{itemize}
    \item Dependence on $K$  and $\alpha$ is $\frac{\sqrt{\log(K)}}{\alpha}$ even when $|B|=0$, which is not as good.
\end{itemize}
